Asymptotic analysis of mixing in stratified turbulent flows, and the conditions for an inertial sub-range

In an important study, Maffioli et al. (J. Fluid Mech., Vol. 794 , 2016) used a scaling analysis to predict that in the weakly stratified flow regime $Fr_h\gg1$ ($Fr_h$ is the horizontal Froude number), the mixing coefficient $\Gamma$ (defined as the ratio of the dissipation rates of potential to kinetic energy) scales as $\Gamma\sim O(Fr_h^{-2})$. Direct numerical simulations confirmed this result, and also indicated that for the strongly stratified regime $Fr_h\ll 1$, $\Gamma\sim O(1)$. Furthermore, the study argued that $\Gamma$ does not depend on the buoyancy Reynolds number $Re_b$, but only on $Fr_h$. We present an asymptotic analysis to predict theoretically how $\Gamma$ should behave for $Fr_h\ll1$ and $Fr_h\gg1$ in the limit $Re_b\to\infty$. To correctly handle the singular limit $Re_b\to\infty$ we perform the asymptotic analysis on the filtered Boussinesq-Navier-Stokes equations, and demonstrate the precise sense in which the inviscid scaling analysis of Billant \& Chomaz (Phys. Fluids, vol. 13, 1645-1651, 2001) applies to viscous flows with $Re_b\to\infty$. The analysis yields $\Gamma\sim O(Fr_h^{-2}(1+Fr_h^{-2}))$ for $Fr_h\gg1$ and $\Gamma\sim O(1+Fr_h^{2})$ for $Fr_h\ll 1$, providing a theoretical basis for the numerical observation made by Maffioli et al, as well as predicting the sub-leading behavior. Our analysis also shows that the Ozmidov scale $L_O$ does not describe the scale below which buoyancy forces are sub-leading, which is instead given by $O(Fr_h^{1/2} L_O)$, and that the condition for there to be an inertial sub-range when $Fr_h\ll 1$ is not $Re_b\gg1$, but the more restrictive condition $Re_b\gg Fr_h^{-4/3}$.

==> table1_inc.tex <==
\begin{tabular}{lrrrrrrrrl}
\toprule
      & $Fr_h$ & $Gn$ & $Re_b$ & $Re_h$              & $N_x $ & $N_z $ & ${\cal L}_x $ & $\epsilon^* / \epsilon_T^*$ & Working name \\ \hline
 run1 &  0.034 &   22 &     69 & $ 5.9 \times 10^4 $ &  14784 &   1840 &             1 &                         1.0 &   F025Gn0014 \\
 run2 &  0.053 &   15 &     60 & $ 2.1 \times 10^4 $ &   6144 &    768 &             1 &                         1.0 &   F035Gn0014 \\
 run3 &  0.094 &   15 &     64 & $ 7.1 \times 10^3 $ &   2048 &    256 &             1 &                         1.0 &   F050Gn0014 \\
 run4 &  0.124 &   16 &     61 & $ 3.9 \times 10^3 $ &   2048 &    256 &             1 &                         1.0 &   F070Gn0014 \\
 run5 &  0.155 &   15 &     50 & $ 2.1 \times 10^3 $ &   2048 &    512 &             1 &                         1.0 &   F100Gn0014 \\
 run6 &  0.257 &   15 &     54 & $ 8.2 \times 10^2 $ &   1024 &    512 &             1 &                         1.0 &   F150Gn0014 \\
 run7 &  0.335 &   16 &     51 & $ 4.5 \times 10^2 $ &    512 &    256 &             1 &                         1.0 &   F200Gn0014 \\
 run8 &  0.449 &   15 &     27 & $ 1.4 \times 10^2 $ &    512 &    512 &             2 &                         1.0 &   F300Gn0014 \\
 run9 &  0.556 &   15 &     23 & $ 7.3 \times 10^1 $ &    256 &    256 &             2 &                         1.0 &   F400Gn0014 \\
run10 &  0.713 &   14 &     21 & $ 4.2 \times 10^1 $ &    128 &    128 &             2 &                         1.0 &   F500Gn0014 \\
\\run11 &  0.027 &   45 &    150 & $ 2.1 \times 10^5 $ &  18432 &   2304 &             1 &                         0.9 &   F025Gn0050 \\
run12 &  0.136 &   82 &    498 & $ 2.7 \times 10^4 $ &   8192 &   1024 &             1 &                         1.0 &   F050Gn0050 \\
run13 &  0.198 &   49 &    196 & $ 5.0 \times 10^3 $ &   4096 &   1024 &             1 &                         1.0 &   F100Gn0050 \\
run14 &  0.404 &   52 &    190 & $ 1.2 \times 10^3 $ &   4096 &   2048 &             1 &                         1.0 &   F200Gn0050 \\
run15 &  0.607 &   44 &    163 & $ 4.4 \times 10^2 $ &    512 &    512 &             2 &                         1.0 &   F400Gn0050 \\
run16 &  0.870 &   51 &    101 & $ 1.3 \times 10^2 $ &    256 &    256 &             2 &                         1.0 &   F600Gn0050 \\
run17 &  1.294 &   50 &     85 & $ 5.1 \times 10^1 $ &    128 &    128 &             2 &                         1.0 &   F800Gn0050 \\
\\run18 &  0.041 &  204 &   1521 & $ 9.1 \times 10^5 $ &  16384 &   2048 &             1 &                         0.2 &   F025Gn0200 \\
run19 &  0.105 &  269 &    542 & $ 5.0 \times 10^4 $ &  14784 &   1848 &             1 &                         1.0 &   F050Gn0200 \\
run20 &  0.209 &  202 &    868 & $ 2.0 \times 10^4 $ &  16384 &   4096 &             1 &                         1.0 &   F100Gn0200 \\
run21 &  0.322 &  207 &    729 & $ 7.0 \times 10^3 $ &   4096 &   2048 &             1 &                         1.0 &   F200Gn0200 \\
run22 &  0.648 &  202 &    689 & $ 1.6 \times 10^3 $ &    512 &    512 &             1 &                         1.0 &   F400Gn0200 \\
run23 &  1.438 &  197 &    521 & $ 2.5 \times 10^2 $ &    512 &    512 &             2 &                         1.0 &   F800Gn0200 \\
run24 &  2.578 &  206 &    443 & $ 6.7 \times 10^1 $ &    256 &    256 &             2 &                         1.0 &  F1600Gn0200 \\
\\run25 &  0.026 & 1278 &   3200 & $ 4.7 \times 10^6 $ &  15840 &   1980 &             1 &                         0.1 &   F025Gn1000 \\
run26 &  0.120 & 2648 &   3447 & $ 2.4 \times 10^5 $ &  14784 &   1848 &             1 &                         0.5 &   F050Gn1000 \\
run27 &  0.210 & 1185 &   2862 & $ 6.5 \times 10^4 $ &  14784 &   3696 &             1 &                         0.7 &   F100Gn1000 \\
run28 &  0.419 & 1368 &   5263 & $ 3.0 \times 10^4 $ &  14784 &   7392 &             1 &                         1.0 &   F200Gn1000 \\
run29 &  0.744 & 1004 &   4662 & $ 8.4 \times 10^3 $ &   3072 &   3072 &             1 &                         0.8 &   F400Gn1000 \\
run30 &  2.078 & 1044 &   5878 & $ 1.4 \times 10^3 $ &   1024 &   1024 &             1 &                         1.0 &   F800Gn1000 \\
run31 &  3.619 & 1066 &   5356 & $ 4.1 \times 10^2 $ &    512 &    512 &             1 &                         1.0 &  F1600Gn1000 \\
\bottomrule
\end{tabular}
